KATO: Knowledge Alignment and Transfer for Transistor Sizing of Different Design and Technology

Automatic transistor sizing in circuit design continues to be a formidable challenge. Despite that Bayesian optimization (BO) has achieved significant success, it is circuit-specific, limiting the accumulation and transfer of design knowledge for broader applications. This paper proposes (1) efficient automatic kernel construction, (2) the first transfer learning across different circuits and technology nodes for BO, and (3) a selective transfer learning scheme to ensure only useful knowledge is utilized. These three novel components are integrated into BO with Multi-objective Acquisition Ensemble (MACE) to form Knowledge Alignment and Transfer Optimization (KATO) to deliver state-of-the-art performance: up to 2x simulation reduction and 1.2x design improvement over the baselines.

==> exp.tex <==

\def\Figref#1{Fig.~\ref{#1}}
\def\Tabref#1{Table~\ref{#1}}
% \newcommand{\YFwrite}[1]{{\color{purple} YF: #1}}


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.75\linewidth]{exp_fig/CASE3.pdf}
  % \vspace*{-0.1in}
  \caption{$P_f$ and FOM on 108-dimensional SRAM column}
  \label{fig:108case}
  % \vspace*{-0.2in}
\end{figure*}
\section{Experimental Results}
\yytodo{Add circuit details, follow the GCN paper}



\cmt
{We firstly examine \ours in five toy examples with different artificial failure boundaries (\eg open boundaries, multiple failure regions, and non-centered regions) with their ground-truth log failure probability (LFP) in \Figref{fig:toy}. Onion sampling with 1000 samples and estimated LFP using kernel density estimator (KDE) with a {bandwidth} of 0.75 are shown in the second row. We can see that onion sampling is efficient but also overestimate the LFP. NSF for the estimated LFP is shown in the third row, which shows significant reductions in the overestimation of onion sampling.

We assess \ours on challenging high-dimensional benchmark circuits, namely, three SRAM column circuits with 108, 569, and 1093 variation parameters, respectively. The circuits are synthesized using the Synopsys Design Compiler and the Cadence Virtuoso design tools.
We set the target failure rate of the circuits at approximately $10^{-5}$ to highlight the challenge of the yield estimation problem.
We implement MC as the golden standard to estimate the ground-truth yields. 
To show the accuracy and efficiency of \ours, we also implement {the} SOTA IS methods, including Minimized Norm Importance Sampling (MNIS) \cite{MNIS}, Hyperspherical Clustering and Sampling (HSCS) \cite{HSCS}, Adaptive Importance Sampling (AIS) \cite{AIS}, Adaptive Clustering and Sampling (ACS) \cite{ACS}, and surrogate-based methods, including Low-Rank Tensor Approximation (LRTA) \cite{LRTA} and Absolute Shrinkage Deep Kernel learning (ASDK) \cite{ASDK}, as comparison methods.

% and then compare \ours with SOTA IS method, including Mnimized Norm Importance Sampling (MNIS) \cite{MNIS}, Hyperspherical Clustering and Sampling (HSCS) \cite{HSCS}, Adaptive Importance Sampling (AIS) \cite{AIS}, Adaptive Clustering and Sampling (ACS) \cite{ACS}, and surrogate-based methods, including Low-Rank Tensor Approximation (LRTA) \cite{LRTA} and Absolute Shrinkage Deep Kernel learning (ASDK) \cite{ASDK}.
% We assess \ours and other SOTA IS- and surrogate-based yield estimation methods to estimate the failure rate and compare their performance.
% The compared competitors includes Mnimized Norm Importance Sampling (MNIS) \cite{MNIS}, Hyperspherical Clustering and Sampling (HSCS) \cite{HSCS}, Adaptive Importance Sampling (AIS) \cite{AIS}, Adaptive Clustering and Sampling (ACS) \cite{ACS}, Low-Rank Tensor Approximation (LRTA) \cite{LRTA} and Absolute Shrinkage Deep Kernel learning (ASDK) \cite{ASDK}. 
% 
% In this section, we also implement ablation experiments to prove that the proposed pre-sampling method does contribute to the performance.   

% In order to determine when to stop the yield estimation algorithm, we choose
The figure of Merit (FOM) $\rho= \mathrm{std}(P_f) / P_f$ (where $\mathrm{std}(P_f)$ is the stand deviation of estimated yield) is used as the stopping criterion for all methods with $\rho=0.1$ (indicating at least 90\% accurate with 90\% confidence interval) as in many previous works, \eg \cite{MNIS, HSCS, AMSV}. 
For the 108-dimensional case, we use a 4-layer multi-layer perception (MLP), each with 432 hidden units; for the high-dimensional 569 and 1093 cases, we use a 7-layer MLP with 600 hidden units for each layer. ReLu activation \cite{relu} is used. The optimization is done with Adam \cite{2014Adam} with 500 epochs. The baseline methods use {(default)} setting as suggested in their papers.
All experiments are performed on a Windows system with AMD 5950x and 32GB RAM.}

\YFwrite{
We commence our evaluation of \ours by considering five illustrative toy examples, each characterized by distinct artificial failure boundaries. These boundaries include scenarios such as open boundaries, multiple failure regions, and non-centered regions. We provide the ground-truth log failure probability (LFP) for these examples in Figure \ref{fig:toy}. The second row of the figure displays the results of onion sampling, which employs 1000 samples and estimates LFP using a kernel density estimator (KDE) \cite{KDE} with a bandwidth of 0.75. It is evident that onion sampling is efficient but tends to overestimate the LFP. To mitigate this overestimation, we introduce a Novel Sampling Framework (NSF), which is presented in the third row. NSF leads to significant reductions in the overestimation observed with onion sampling.

Moving on to more challenging high-dimensional benchmark circuits, we focus on three SRAM column circuits, each characterized by a different number of variation parameters (108, 569, and 1093, respectively). These circuits are synthesized using the Synopsys Design Compiler and the Cadence Virtuoso design tools. We set the target failure rate of these circuits at approximately $10^{-5}$ to emphasize the difficulty of the yield estimation problem. To establish a benchmark for comparison, we implement MC as the gold standard for estimating ground-truth yields.
In addition to \ours, we also implement several SOTA IS-based methods, including Minimized Norm Importance Sampling (MNIS) \cite{MNIS}, Hyperspherical Clustering and Sampling (HSCS) \cite{HSCS}, Adaptive Importance Sampling (AIS) \cite{AIS}, and Adaptive Clustering and Sampling (ACS) \cite{ACS}. Furthermore, we employ surrogate-based methods such as Low-Rank Tensor Approximation (LRTA) \cite{LRTA} and Absolute Shrinkage Deep Kernel Learning (ASDK) \cite{ASDK} for comparison purposes.

We evaluate the methods using the Figure of Merit (FOM) $\rho = \mathrm{std}(P_f) / P_f$, where $\mathrm{std}(P_f)$ represents the standard deviation of estimated yields. A stopping criterion of $\rho = 0.1$ is applied, indicating that we aim for at least 90\% accuracy with a 90\% confidence interval. This criterion aligns with established practices in previous works such as \cite{MNIS, HSCS, AMSV}.

For the 108-dimensional case, we employ a 4-layer multi-layer perceptron (MLP) \cite{MLP} with 432 hidden units in each layer. For the high-dimensional 569 and 1093 cases, we opt for a 7-layer MLP, with each layer containing 600 hidden units. Rectified Linear Unit (ReLU) activation functions \cite{relu} are used throughout. The optimization process employs the Adam optimizer \cite{2014Adam} and runs for 500 epochs. 
The baseline methods are implemented using their default settings, adhering to the recommendations outlined in their respective papers. In situations where specific methods exhibit limited generalization, we conduct hyperparameter fine-tuning to optimize performance across various experimental scenarios.
All experiments are conducted on a Windows system equipped with an AMD 5950x processor and 32GB of RAM.
}



\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{exp_fig/sram_array.pdf}
  % \vspace*{-0.1in}
  \caption{The structure of SRAM column circuit}
  \label{SRAM_column}
  % \vspace*{-0.2in}
\end{figure}





% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{paper_fig/108dim.pdf}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{paper_fig/1093dim.pdf}
%          \caption{$y=3\sin x$}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{paper_fig/1093dim.pdf}
%          \caption{$y=5/x$}
%          \label{fig:five over x}
%      \end{subfigure}
%         \caption{Three simple graphs}
%         \label{fig:three graphs}
% \end{figure}

% \begin{figure}[ht]
%   \centering

%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{image1}
%     \caption{图1}
%     \label{fig:subfig1}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{image2}
%     \caption{图2}
%     \label{fig:subfig2}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.32\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{image3}
%     \caption{图3}
%     \label{fig:subfig3}
%   \end{subfigure}

%   \caption{三张图片并排显示}
%   \label{fig:mainfig}
% \end{figure}

% \begin{figure*}[]
%   \centering
%   \begin{subfigure}{0.33\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{paper_fig/108dim.pdf}
%     \caption{OTA}
%     \label{fig:OTA}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.33\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{paper_fig/569dim.pdf}
%     \caption{6T-SRAM}
%     \label{fig:6T-SRAM}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.33\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{paper_fig/569dim.pdf}
%     \caption{Adder}
%     \label{fig:Adder}
%   \end{subfigure}
%   \vspace*{-0.05in}
%   \caption{Yield optimization for the three circuits with different numbers of total simulations}
%   \label{fig:three_images}
% \end{figure*}
 
 % \help{experimental setting: dense network}

% to indicates a estimation of 
% to terminated the iteratio
% we stop the process of yield estimation and declare that the estimated $P_f$ is 



% \begin{table*}
%   \centering
%       \tabcolsep=5pt
%       \caption{Numerical results on three SRAM column circuits}
%       \label{AllCaseTable}
%       \vspace*{-0.1in}
%       \begin{tabular}{l|cccc|cccc|cccc}
%         \toprule
%         & \multicolumn{4}{|c|}{108-dimensional case} & \multicolumn{4}{|c|}{569-dimensional case}  & \multicolumn{4}{|c}{1093-dimensional case} \\
%         \midrule
%          Method & Fail. prob. & Rel. error & \# of sim. & Speedup & Fail. prob. & Rel. error & \# of sim. & Speedup & Fail. prob. & Rel. error & \# of sim. & Speedup\\
%         \midrule
%         MC   & 5.01e-5 &   -   & 699000 & 1x & 2.50e-5 &   -   & 931000 & 1x & 4.80e-5 &   -   & 1189000 & 1x \\
%         MNIS & 4.15e-5 & 17.07\% & 47500 & 14.72x & 2.07e-5 & 17.33\% & 59000  & 15.78x & 4.21e-5 & 12.32\% & 81000 & 14.68x\\
%         HSCS & 4.84e-5 & 3.36\% & 26500 & 26.38x & 2.86e-5 & 14.27\% & 46500  & 20.02x & 4.30e-5 & 10.47\% & 66000 & 18.02x\\
%         AIS  & 4.75e-5 & 5.21\% & 12300 & 56.83x & 2.38e-5 & 4.99\%  & 25700  & 36.23x & 4.43e-5 & 7.75\% & 38000 & 31.29x\\
%         ACS  & 5.68e-5 & 13.40\% & 10400 & 67.21x & 2.73e-5 & 9.19\%  & 22500  & 41.38x & 4.42e-5 & 7.83\% & 30400 & 39.11x\\
%         LRTA & 4.50e-5 & 10.18\% & 13000 & 53.77x & 2.26e-5 & 9.60\%  & 18500  & 50.32x & 5.25e-5 & 9.38\% & 24000 & 49.54x\\
%         ASDK & 4.5e-5 & 10.18\% & 9200 & 75.98x & 2.30e-5 & 8.00\% & 11800 & 78.90x & 6.10e-5 & 27.08\% & 14550 & 81.72x\\
%         Proposed & 5.02e-5 & \bf{0.21}\% & \bf{5300} & \bf{131.89x} & 2.49e-5 & \bf{0.25}\% & \bf{3400} & \bf{273.82x} & 4.67e-5 & \bf{2.71}\% & \bf{6400} & \bf{185.78x}\\
%       \bottomrule
%     \end{tabular}
%     \vspace*{-0.1in}
% \end{table*}
% \begin{table*}
%   \centering
%       % \tabcolsep=5pt
%       \caption{Numerical results on three SRAM column circuits}
%       \label{AllCaseTable}
%       % \vspace*{-0.1in}
%       \begin{adjustbox}{width=2.1\columnwidth,center}
%       \renewcommand\arraystretch{1.3}
%       \setlength{\tabcolsep}{2.2pt}
%       \begin{tabular}{l|cccc|cccc|cccc}
%         \toprule[1.5pt]
%         & \multicolumn{4}{c|}{108-dimensional case} & \multicolumn{4}{c|}{569-dimensional case}  & \multicolumn{4}{c}{1093-dimensional case} \\
%         \midrule
%         Method & Fail. prob. & Rel. error & \#Sim. & Speedup & Fail. prob. & Rel. error & \#Sim. & Speedup & Fail. prob. & Rel. error & \#Sim. & Speedup\\
%         \midrule[1pt]
%         MC   & 5.01e-5 &   -   & 699000 & 1x & 2.50e-5 &   -   & 931000 & 1x & 4.80e-5 &   -   & 1189000 & 1x \\
%         MNIS & 4.15e-5 & 17.07\% & 47500 & 14.72x & 2.07e-5 & 17.33\% & 59000  & 15.78x & 4.21e-5 & 12.32\% & 81000 & 14.68x\\
%         HSCS & 4.85e-5 & 9.59\% & 36700 & 19.05x & 1.63e-5 & 34.80\% & 63600  & 14.64x & 1.53e-6 & Error & 95580 & 12.44x\\
%         AIS  & 4.92e-5 & 1.79\% & 18000 & 38.83x & 2.63e-5 & 5.20\%  & 22800  & 40.83x & 3.79e-5 & 21.04\% & 27900 & 42.62x\\
%         ACS  & 4.95e-5 & 1.19\% & 11540 & 60.57x & 2.39e-5 & 4.40\%  & 18100  & 51.44x & 4.30e-5 & 10.42\% & 24000 & 49.54x\\
%         LRTA & 4.86e-5 & 2.99\% & 10550 & 63.41x & 2.21e-5 & 11.60\%  & 13500  & 68.96x & 3.33e-5 & 30.63\% & 21000 & 56.61x\\
%          ASDK & 4.68e-5 & 6.59\% & 9500 & 73.57x & 2.05e-5 & 18.00\% & 10500 & 78.90x & 3.51e-5 & 26.87\% & 18000 & 66.05x\\
%         Proposed & 5.00e-5 & \bf{0.21}\% & \bf{4345} & \bf{160.87x} & 2.49e-5 & \bf{0.25}\% & \bf{4883} & \bf{190.66x} & 4.95e-5 & \bf{3.13}\% & \bf{4832} & \bf{246.01x}\\
%       \bottomrule[1.5pt]
%     \end{tabular}
%     % \vspace*{-0.1in}
%     \end{adjustbox}
% \end{table*}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.75\linewidth]{exp_fig/CASE4.pdf}
  % \vspace*{-0.1in}
  \caption{$P_f$ and FOM on 569-dimensional SRAM column}
  \label{fig:569case}
  % \vspace*{-0.2in}
\end{figure}

\subsection{108-Dimensional SRAM Column Circuit} \label{108dim_exp}



% \begin{table}
%   \vspace{-0.15in}
%   \centering
%   \caption{nOCR on 108-dimensional SRAM column}
%   \label{robustness}
%   \vspace{-0.1in}
%     \begin{adjustbox}{width=1\columnwidth,center}
%     \renewcommand\arraystretch{1.2}
%       \setlength{\tabcolsep}{2.5pt}
%       \begin{tabular}{c|cccccccc}
%         \toprule[1.5pt]
%          Method & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%         \midrule[1pt]
%          nOCR  & 507.4 & 198.6 & 2169.3 & 5089.9  & 528.2 & 746.4 & \bf{62804.7} \\
%          nOCR(norm) & 8.08e-3 & 3.16e-3 & 3.45e-2 & 8.10e-2 & 8.41e-3 & 1.19e-2 & \bf{1} \\    
%       \bottomrule[1.5pt]
%     \end{tabular}
% \end{adjustbox}
% % \vspace*{-0.1in}
% \end{table}

\cmt{
An SRAM array is a typical type of random-access memory and uses flip-flop{s} to store data. The SRAM array and cell are shown in \Figref{SRAM_column}, where WL is the word line, and BL is the bit line; two cross-connected inventors composed of four transistors are used for storing data, whereas the other two transistors work as control switches for data transmission.
Each transistor contains three variational parameters.
An 8-bit SRAM array is composed of eight cells, resulting in 108 variation parameters. We choose the delay time of read/write of the SRAM as the output performance metric $\y$ of the circuit. 
}
\cmt
{An SRAM array is a common form of random-access memory that utilizes flip-flops for data storage. The architecture of the SRAM array and its cells is depicted in \Figref{SRAM_column}, where “WL” represents the word line and “BL” represents the bit line. The storage of data employs two cross-connected inverters, each consisting of four transistors, while the remaining two transistors function as control switches for data transmission.
It is worth noting that each transistor comprises three distinct variational parameters. In the context of an 8-bit SRAM array composed of eight cells, this yields a total of 108 variation parameters. As a performance metric for the circuit, we select the read/write delay time of the SRAM operations, denoted as output performance metric $\y$.}
%  Our experiment is implemented on a SRAM column circuit with And 
% We compare different methods (MC, MNIS, HSCS, AIS, ACS, LRTA, ASDK, proposed) in accuracy and efficiency.


% In terms of accuracy, 
\cmt
{We show the failure probability estimation and FOM in \Figref{fig:108case}, and the numerical results are concluded in \Tabref{table:108Case}.
The advantage of \ours is obvious by giving a 131.89x speedup compared to MC, more than twice faster {than} the second-best method AIS. Except for being the fastest, \ours also achieves the best accuracy among all methods with a relative error of 0.21\%, more than 10x better than the second-best method HSCS. It is also interesting to see that \ours seriously overestimates the failure due to the suboptimal onion sampling. Such a bias is then sequentially reduced as more samples are collected.}
\cmt
{We present the estimation of failure probability and FOM in \Figref{fig:108case}, while the numerical outcomes are summarized in \Tabref{table:108Case}. The evident advantage of \ours becomes apparent, showcasing a remarkable speedup of 131.89 times when compared to the traditional Monte Carlo (MC) approach. This substantial acceleration surpasses even the second-best technique, AIS, by more than a twofold margin. In addition to its superior speed, \ours attains the highest level of accuracy across all methods, exhibiting a relative error of merely 0.21\%, surpassing the second-best contender, HSCS, by over tenfold.
It is noteworthy that the performance of \ours tends to exhibit an overestimation of failure probabilities due to the inherent suboptimal nature of onion sampling. However, this bias progressively diminishes as the accumulation of samples advances, aligning the estimates with enhanced accuracy.}

\YFwrite{

An SRAM array is a widely used form of random-access memory that employs flip-flops to store data. The architecture of the SRAM array and its individual cells is illustrated in \Figref{SRAM_column}. In this diagram, “WL” represents the word line, and “BL” represents the bit line. Data storage is achieved through the use of two cross-connected inverters in each cell, with each inverter comprising four transistors. Additionally, the remaining two transistors are utilized as control switches to facilitate data transmission.
It's important to note that each transistor within the SRAM cell is characterized by three distinct variational parameters. In the context of an 8-bit SRAM array, consisting of eight individual cells, this results in a total of 108 variation parameters that need to be considered. To assess the performance of the circuit, we focus on the read/write delay time of SRAM operations, which is denoted as the output performance metric $\y$.

We present the estimation of failure probability and the FOM in Figure \ref{fig:108case}, and the numerical results are summarized in Table \ref{table:108Case}. The remarkable advantage of \ours is readily apparent, demonstrating an impressive speedup of 131.89 times when compared to the conventional MC approach. This substantial acceleration surpasses even the second-best technique, AIS, by more than a twofold margin.
In addition to its exceptional speed, \ours achieves the highest level of accuracy among all methods, with a relative error of only 0.21\%. This surpasses the second-best method, HSCS, by more than tenfold. It's worth noting that the performance of \ours may initially exhibit an overestimation of failure probabilities due to the suboptimal nature of onion sampling. However, this bias gradually diminishes as more samples are accumulated, resulting in estimates that align with enhanced accuracy.

}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.75\linewidth]{exp_fig/CASE5.pdf}
  % \vspace*{-0.1in}
  \caption{$P_f$ and FOM on 1093-dimensional SRAM column}
  \label{fig:1093case}
  % \vspace*{-0.2in}
\end{figure*}

\subsection{569-Dimensional SRAM Column Circuit}


\begin{table}[h]
\centering
\caption{Results on 108-dimensional SRAM circuit}
\label{table:108Case}
      % \vspace*{-0.1in}
      \begin{adjustbox}{width=1\columnwidth,center}
      \renewcommand\arraystretch{1.6}
      \setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l|ccccc}
% \hline
\toprule[1.5pt]
\toprule
Method & Fail Rate & Rel. Error & \# Sim & Speedup & nACR \\ 
\midrule[1pt]
% \hline
MC & 5.01e-5 & - & 699000 & 1x & - \\
MNIS & 4.15e-5 & 17.07\% & 47500 & 14.72x & 0.08x \\
HSCS & 4.85e-5 & 9.59\% & 36700 & 19.05x & 0.11x \\
AIS & 4.92e-5 & 1.79\% & 18000 & 38.83x & 0.24x \\
ACS & 4.95e-5 & 1.19\% & 11540 & 60.57x & 0.37x \\
LRTA & 4.86e-5 & 2.99\% & 10550 & 63.41x & 0.30x \\
ASDK & 4.68e-5 & 6.59\% & 9500 & 73.57x & 0.43x \\
Proposed & \textbf{5.00e-5} & \textbf{0.21\%} & \textbf{4345} & \textbf{160.87x} & \textbf{1.00x} \\ 
% \hline
\bottomrule
\bottomrule[1.5pt]
\end{tabular}
\end{adjustbox}
\end{table}

% \begin{figure*}[t]
%   \centering
%   %minipage
%   % \begin{minipage}[t]{1\linewidth}
%     % \centering
%     % \vspace*{-0.1in}
%     \includegraphics[width=0.8\linewidth]{exp_fig/case3_Pfail.pdf}\\
%     \vspace{-0.1in}
%     \includegraphics[width=0.8\linewidth]{exp_fig/case3_FOM.pdf}\\
%     % \vspace{-0.1in}
%     \caption{$P_f$ and FOM on 108-dimensional SRAM column}
%     \label{case4_exp}
%   % \end{minipage}
%   % \vspace{-0.2in}
% \end{figure*}



% \begin{figure}
%   \centering
%   \includegraphics[width=1\linewidth]{exp_fig/108dim_error.pdf}
%   % \vspace*{-0.1in}
%   \caption{The structure of SRAM column circuit}
%   \label{SRAM_column}
%   % \vspace*{-0.2in}
% \end{figure}

% \begin{figure}[h]
% % \vspace*{-0.1in}
%   \centering
%   \includegraphics[width=0.88\linewidth]{paper_fig/108dim.pdf}
%   % \vspace*{-0.05in}
%   \caption{nACR on 108-dimensional SRAM circuit}
%   \label{fig:warp}
%   % \vspace*{-0.1in}
% \end{figure}

% \begin{figure}[h]
%   \centering
% 	\includegraphics[width=1\linewidth]{exp_fig/case3_Pfail.pdf}\\
% 	\vspace{-0.1in}
% 	\includegraphics[width=1\linewidth]{exp_fig/case3_FOM.pdf}\\
%   % \vspace{-0.1in}
%   \caption{$P_f$ and FOM on 108-dimensional SRAM column}
%   \label{case3_exp}
%   % \vspace{-0.1in}
% \end{figure}

% The ground truth of failure rate by the MC method is 5.01e-5, using 699k runs of simulation. And It can be seen that \ours outperforms all other competitors in terms of estimation accuracy and convergence efficiency of achieving a steady state, exhibiting only a 0.21\% relative error and 131.89x speedup to the MC. 
% \ours uses 5300 simulation runs to achieve convergence, while MNIS, HSCS, AIS, ACS, LRTA and ASDK consumes 47.5k, 26.5k, 12.3k, 10.4k, 13k and .... simulation runs respectively.   
% The $P_f$ of IS-based approaches like MNIS, HSCS, AIS and ACS remains very low at the first half of the evolution, because they don't find enough failure regions. When they find a correct failure region, a sudden increase in $p_f$ arises and it will finally converge to the MC ground truth result. AIS and ACS render faster convergence than MNIS and HSCS, because ACS and AIS are able to adaptively discover failure regions while searching areas of MNIS and HSCS are pre-fixed. 
% The $P_f$ evolution of surrogate-based methods like LRTA and ASDK is majorly determined by the model fitting accuracy to the variation parameter space. With enough training data, $P_f$ of surrogate-based methods converges to the ground truth. 
% \ours outperforms all other IS-based competitors because they need a large number of pre-sampling and \ours's novel adaptive scheme speeds up the convergence efficiency.  \ours outperforms all other surrogate-based competitors because surrogate methods need large number of training data to achieve an accurate model due to the ``curse of dimensionality''. 







% \begin{table*}
% \centering
%     \caption{Numerical results on 569-dimensional SRAM column}
%     \begin{tabular}{c|c|cccccccc}
%       \toprule
%        & Results & MC & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%       \midrule
      
%       \multirow{4}{*}{Successful runs} 
%       & Mean failure prob.   & 2.50e-5 & 2.34e-5 & 2.68e-5 & 2.31e-5 & 2.69e-5 & 2.29e-5 &  & 2.58e-5\\
%       & Mean relative error  & Golden & 6.29\% & 7.13\% & 7.61\% & 7.80\%  & 8.48\% &  & 3.41\% \\
%       & Mean \# of sim.      & 931000.00 & 69816.66 & 49975.00 & 28500.00 &  24812.50  & 19430.00  &  & 3600.00 \\
%       & Mean speedup & 1x & 13.33x & 18.63x & 32.67x & 37.52x & 47.92x & & 258.61x \\
%      \midrule
    
%      \multirow{1}{*}{Failed runs} 
%       & Failed times & N/A & 4/10 & 2/10 & 3/10 & 2/10 & 5/10 &  & 2/10 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}




% \begin{table*}
% \centering
%     \caption{Numerical results on 1093-dimensional SRAM column}
%     \begin{tabular}{c|c|cccccccc}
%       \toprule
%        & Results & MC & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%       \midrule
      
%       \multirow{4}{*}{Successful runs} 
%       & Mean failure prob.   & 4.80e-5 & 4.51e-5 & 4.50e-5 & 4.59e-5 & 5.08e-5 & 5.30e-5 &  & 4.84e-5\\
%       & Mean relative error  & Golden & 6.09\% & 6.22\% & 4.43\% & 5.91\%  & 10.41\% &  & 0.73\% \\
%       & Mean \# of sim.      & 1189000.00 & 88928.57 & 72500.00 & 40557.14  & 35628.57  & 25125.00   &  &  6600.00\\
%       & Mean speedup & 1x & 13.37x & 16.40x & 29.32x & 33.37x & 47.32x & & 180.15x \\
%      \midrule
    
%      \multirow{1}{*}{Failed runs} 
%       & Failed times & N/A & 3/10 & 4/10 & 3/10 & 3/10 & 6/10 &  & 2/10 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}


% \begin{figure}[H]
% 	\includegraphics[width=1\linewidth]{exp_fig/case4_Pfail.pdf}
% 	\includegraphics[width=1\linewidth]{exp_fig/case4_FOM.pdf}
%     \caption{Best run of $P_f$  and FOM on 569-dimensional SRAM column}
%   \label{case4_exp}
% \end{figure}



% \end{figure}
% \begin{figure}[H]
% 	\includegraphics[width=1\linewidth]{exp_fig/case5_Pfail.pdf}
% 	\includegraphics[width=1\linewidth]{exp_fig/case5_FOM.pdf}

%     \caption{ Best run of $P_f$  and FOM on 1093-dimensional SRAM column}
%   \label{case5_exp}
% \end{figure}



% 合并图表
% \begin{table*}
% \centering
%     \tabcolsep=4pt
%     \caption{Numerical results on three SRAM column circuits}
%     \label{AllCaseTable}
%     \begin{tabular}{c|cccc|cccc|cccc}
%       \toprule
%       & \multicolumn{4}{|c|}{108-dimensional circuit case} & \multicolumn{4}{|c|}{569-dimensional circuit case}  & \multicolumn{4}{|c}{1093-dimensional circuit case} \\
%       \midrule
%        Method & Fail. prob. & Rel. error & \# of sim. & Speedup & Fail. prob. & Rel. error & \# of sim. & Speedup & Fail. prob. & Rel. error & \# of sim. & Speedup\\
%       \midrule
%       MC   & 5.01e-5 &   N/A   & 699000 & 1x & 2.50e-5 &   N/A   & 931000 & 1x & 4.80e-5 &   N/A   & 1189000 & 1x \\
%       MNIS & 4.15e-5 & 17.07\% & 47500 & 14.72x & 2.07e-5 & 17.33\% & 59000  & 15.78x & 4.21e-5 & 12.32\% & 81000 & 14.68x\\
%       HSCS & 4.84e-5 & 3.36\% & 26500 & 26.38x & 2.86e-5 & 14.27\% & 46500  & 20.02x & 4.30e-5 & 10.47\% & 66000 & 18.02x\\
%       AIS  & 4.75e-5 & 5.21\% & 12300 & 56.83x & 2.38e-5 & 4.99\%  & 25700  & 36.23x & 4.43e-5 & 7.75\% & 38000 & 31.29x\\
%       ACS  & 5.68e-5 & 13.40\% & 10400 & 67.21x & 2.73e-5 & 9.19\%  & 22500  & 41.38x & 4.42e-5 & 7.83\% & 30400 & 39.11x\\
%       LRTA & 4.50e-5 & 10.18\% & 13000 & 53.77x & 2.26e-5 & 9.60\%  & 18500  & 50.32x & 5.25e-5 & 9.38\% & 24000 & 49.54x\\
%       ASDK & e-5 & \% &  & x & 2.30e-5 & 8.00\% & 11800 & 78.90x & 6.10e-5 & 27.08\% & 14550 & 81.72x\\
%       Proposed & 5.02e-5 & 0.21\% & 5300 & 131.89x & 2.49e-5 & 0.25\% & 3400 & 273.82x & 4.67e-5 & 2.71\% & 6400 & 185.78x\\
%     \bottomrule
%   \end{tabular}
% \end{table*}



% 独次最好的结果
% \begin{table}
% \centering
%     \caption{Best numerical results on 108-dimensional SRAM column}
%     \label{case3Table}
%     \begin{tabular}{c|cccc}
%       \toprule
%       Method & Failure prob. & Relative error & \# of sim. & Sim. speedup\\
%       \midrule
%       MC   & 5.01e-5 &   N/A   & 699000 & 1x\\
%       MNIS & 4.15e-5 & 17.07\% & 47500 & 14.72x\\
%       HSCS & 4.84e-5 & 3.36\% & 26500 & 26.38x\\
%       AIS  & 4.75e-5 & 5.21\% & 12300 & 56.83x\\
%       ACS  & 5.68e-5 & 13.40\% & 10400 & 67.21x\\
%       LRTA & 4.50e-5 & 10.18\% & 13000 & 53.77x\\
%       ASDK & e-5 & \% &  & x\\
%       Proposed & 5.02e-5 & 0.21\% & 5300 & 131.89x\\
%     \bottomrule
%   \end{tabular}
%   \end{table}

% \begin{table}
% \centering
%     \caption{Best numerical results on 569-dimensional SRAM column}
%     \label{case4Table}
%     \begin{tabular}{c|cccc}
%       \toprule
%       Method & Failure prob. & Relative error & \# of sim. & Sim. speedup\\
%       \midrule
%       MC       & 2.50e-5 &   N/A   & 931000 & 1x\\
%       MNIS     & 2.07e-5 & 17.33\% & 59000  & 15.78x\\
%       HSCS     & 2.86e-5 & 14.27\% & 46500  & 20.02x\\
%       AIS      & 2.38e-5 & 4.99\%  & 25700  & 36.23x\\
%       ACS      & 2.73e-5 & 9.19\%  & 22500  & 41.38x\\
%       LRTA     & 2.26e-5 & 9.60\%  & 18500  & 50.32x\\
%       ASDK     & e-5 & \% &  & x\\
%       Proposed & 2.49e-5 & 0.25\% & 3400 & 273.82x\\
%     \bottomrule
%   \end{tabular}
%   \end{table}

% \begin{table}
% \centering
%     \caption{Best numerical results on 1093-dimensional SRAM column}
%     \label{case5Table}
%     \begin{tabular}{c|cccc}
%       \toprule
%       Method & Failure prob. & Relative error & \# of sim. & Sim. speedup\\
%       \midrule
%       MC       & 4.80e-5 &   N/A   & 1189000 & 1x \\
%       MNIS     & 4.21e-5 & 12.32\% & 81000 & 14.68x\\
%       HSCS     & 4.30e-5 & 10.47\% & 66000 & 18.02x\\
%       AIS      & 4.43e-5 & 7.75\% & 38000 & 31.29x\\
%       ACS      & 4.42e-5 & 7.83\% & 30400 & 39.11x\\
%       LRTA     & 5.25e-5 & 9.38\% & 24000 & 49.54x\\
%       ASDK     & e-5 & \% &  & x\\
%       Proposed & 4.67e-5 & 2.71\% & 6400 & 185.78x\\
%     \bottomrule
%   \end{tabular}
%   \end{table}


% YF的图

% \begin{figure}
%     \caption{pre-sampling}
%   \label{case7_exp}
% \end{figure}

% \begin{figure}

%     \caption{nf}
%   \label{case8_exp}
% \end{figure}


% \begin{table*}
% \centering
%     \caption{Ablation experiment of pre-sampling method}
%     \begin{tabular}{c|c|c|c|c}
%       \toprule
%          & 1 & 2 & 3 & 4  \\
%        \midrule
%         Target density& \includegraphics[width=0.18\textwidth]{paper_fig/fig_2.jpeg}&  \includegraphics[width=0.2\textwidth]{paper_fig/fig_3.jpeg}  & \includegraphics[width=0.2\textwidth]{paper_fig/fig_5.jpeg} & \\
%       \midrule
%               Pre-sampling  & \includegraphics[width=0.2\textwidth]{paper_fig/pre_2.png} & \includegraphics[width=0.2\textwidth]{paper_fig/pre_3.png} & \includegraphics[width=0.2\textwidth]{paper_fig/pre_4.png} &  \\
%        \midrule
%                Nf-sample & \includegraphics[width=0.2\textwidth]{paper_fig/nf_2.png} & \includegraphics[width=0.2\textwidth]{paper_fig/nf_3.png} & \includegraphics[width=0.2\textwidth]{paper_fig/nf_4.png} &  \\
%         \midrule
%                 Flow density
%     \bottomrule
%   \end{tabular}
% \end{table*}



% \begin{table}
%   \vspace{-0.15in}
%   \centering
%   \caption{nOCR on 569-dimensional SRAM column}
%   \label{robustness}
%   \vspace{-0.1in}
%     \begin{adjustbox}{width=1\columnwidth,center}
%     \renewcommand\arraystretch{1.2}
%       \setlength{\tabcolsep}{2.5pt}
%       \begin{tabular}{c|cccccccc}
%         \toprule[1.5pt]
%          Method & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%         \midrule[1pt]
%          nOCR  & 165.3 & 40.1 & 785.2 & 1169.1  & 524.2 & 986.3 & \bf{109528} \\
%         % & Mean \# of sim.      & 699000.00 & 50883.33 & 31340.00 & 15714.29 & 14071.43   & 13440.00  &  & 5300.00 \\
%          nOCR(norm) & 1.51e-3 & 3.66e-4 & 7.17e-3 & 1.07e-2 & 4.78e-3 & 9.01e-3 & \bf{1} \\   
%       \bottomrule[1.5pt]
%     \end{tabular}
% \end{adjustbox}
% % \vspace*{-0.1in}
% \end{table}
\cmt
{To validate \ours in practical scenarios, we work on a commercial SRAM array solution with 528 transistors in the design to form bit-cell arrays, sense amplifiers, and power paths. Based on the transistor type (PMOS/NMOS), gate length, and gate width, each transistor will associate with 0-3 variational parameters (\ie mobility, oxide thickness, and saturation velocity) based on the BSIM model.
With a BSIM4 model, this leads to 569 variation parameters. }
\cmt
{For the purpose of practical validation, we apply \ours to a real-world scenario involving a commercial SRAM array solution comprising a total of 528 transistors. This solution encompasses the creation of bit-cell arrays, sense amplifiers, and power paths. Taking into account the transistor's characteristics, such as type (PMOS/NMOS), gate length, and gate width, each transistor corresponds to 0 to 3 distinct variational parameters, namely mobility, oxide thickness, and saturation velocity, as stipulated by the BSIM model.
Employing the BSIM4 model in this context engenders a cumulative count of 569 variation parameters.
% where each transistor instance is instantiated based on a model and instantiation parameters, such as the transistor type (PMOS/NMOS), the gate length, and the gate width, and each transistor has a random number between 0 and 3 associated with it. 
% The random numbers correspond to various parameters that affect the transistor behavior, such as mobility, oxide thickness, saturation velocity, etc.
% we further increase the number of SRAM bit cells in the SRAM column, which leads to an SRAM circuit with 569 variation parameters. 
The delay time of read/write of the SRAM acts as the output metric $\y$. }
% We run the same yield estimation algorithm on the 569-dimensional circuit.
\cmt
{The convergence dynamic is shown in \Figref{fig:569case} with results in \Tabref{tab:569}.
Similarly, the results of \ours are significantly better than the competitors, showing a 273.82x speedup over MC, which is almost 3.5x faster than the second-best method ASDK. Most importantly, the estimation results are very close to the ground truth, with a relative error of 0.25\%. Again, the initial overestimation remains for \ours.}
\cmt
{The progression of convergence is depicted in Figure \ref{fig:569case}, accompanied by the outcomes summarized in Table \ref{tab:569}.
Consistently echoing the trend observed earlier, the performance of \ours continues to outshine its competitors. This time, it showcases an astounding acceleration, boasting a speedup of 273.82 times when compared to the MC methodology. This swiftness is nearly 3.5 times quicker than the second-ranking contender, ASDK. Of paramount significance, the estimates produced by \ours maintain remarkable proximity to the actual ground truth, exhibiting a mere relative error of 0.25%.
As observed previously, it is noteworthy that \ours initially tends to overestimate failure probabilities, a trait stemming from the inherent nature of the onion sampling technique. However, akin to the prior cases, this tendency gradually fades as more samples are assimilated, leading to progressively refined estimations.}

\YFwrite{
To validate the practical applicability of \ours, we apply it to a real-world scenario involving a commercial SRAM array solution. This SRAM array comprises a total of 528 transistors and encompasses the creation of bit-cell arrays, sense amplifiers, and power paths.
Each transistor in this solution is characterized by specific attributes, including its type (PMOS/NMOS), gate length, and gate width. Furthermore, each transistor corresponds to 0 to 3 distinct variational parameters, which include mobility, oxide thickness, and saturation velocity, as dictated by the BSIM model.
In this context, employing the BSIM4 model leads to a cumulative count of 569 variation parameters. We focus on evaluating the delay time associated with read and write operations of the SRAM, which serves as the output metric $\y$. This practical validation allows us to assess the performance and effectiveness of \ours in a real-world scenario involving a complex SRAM array design.

The convergence progress is illustrated in Figure \ref{fig:569case}, and the results are summarized in Table \ref{tab:569}. In line with the previous observations, the performance of \ours consistently outperforms its competitors. This time, it demonstrates an impressive acceleration, achieving a remarkable speedup of 273.82x when compared to the traditional MC methodology. This rapidity is nearly 3.5 times faster than the second-best method, ASDK.
Of utmost significance, the estimates produced by \ours remain exceptionally close to the actual ground truth, displaying a mere relative error of 0.25\%.
As noted previously, it's worth mentioning that \ours may initially exhibit a tendency to overestimate failure probabilities, a characteristic stemming from the inherent nature of the onion sampling technique. However, as observed in earlier cases, this tendency gradually diminishes as more samples are collected, resulting in increasingly refined estimations.
}

\begin{table}[h]
\centering
\caption{Results on 569-dimensional SRAM circuit}
\label{tab:569}
      % \vspace*{-0.1in}
      \begin{adjustbox}{width=1\columnwidth,center}
      \renewcommand\arraystretch{1.6}
      \setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l|ccccc}
% \hline
\toprule[1.5pt]
\toprule
Method & Fail Rate & Rel. Error & \# Sim & Speedup & nACR \\ 
\midrule[1pt]
% \hline
MC & 2.50e-5 & - & 931000 & 1x & - \\
MNIS & 2.07e-5 & 17.33\% & 59000 & 15.78x & 0.07x \\
HSCS & 1.63e-5 & 34.80\% & 63600 & 14.64x & 0.05x \\
AIS & 2.63e-5 & 5.20\% & 22800 & 40.83x & 0.20x \\
ACS & 2.39e-5 & 4.40\% & 18100 & 51.44x & 0.26x \\
LRTA & 2.21e-5 & 11.60\% & 13500 & 68.96x & 0.24x \\
ASDK & 2.05e-5 & 18.00\% & 10500 & 78.90x & 0.38x \\
Proposed & \textbf{2.49e-5} & \textbf{0.25\%} & \textbf{4883} & \textbf{190.66x} & \textbf{1.00x} \\
% \hline
\bottomrule
\bottomrule[1.5pt]
\end{tabular}
\end{adjustbox}
\end{table}

% \begin{figure}[h]
% % \vspace*{-0.1in}
%   \centering
%   \includegraphics[width=0.88\linewidth]{paper_fig/569dim.pdf}
%   % \vspace*{-0.05in}
%   \caption{nACR on 569-dimensional SRAM circuit}
%   \label{fig:warp}
%   % \vspace*{-0.1in}
% \end{figure}

% \begin{figure*}[t]
%   \centering
%   %minipage
%   % \begin{minipage}[t]{1\linewidth}
%     % \centering
%     % \vspace*{-0.1in}
%     \includegraphics[width=0.8\linewidth]{exp_fig/case4_Pfail.pdf}\\
%     \vspace{-0.1in}
%     \includegraphics[width=0.8\linewidth]{exp_fig/case4_FOM.pdf}\\
%     % \vspace{-0.1in}
%     \caption{$P_f$ and FOM on 569-dimensional SRAM column}
%     \label{case4_exp}
%   % \end{minipage}
%   % \vspace{-0.2in}
% \end{figure*}



% \begin{table}[t]
% \centering
% % \vspace{-0.1in}
%   \centering
%   \caption{nACR on three SRAM circuits}
%   \label{robustness}
%   % \vspace{-0.1in}
% \begin{adjustbox}{width=1\columnwidth,center}
%     \renewcommand\arraystretch{1.5}
%       \setlength{\tabcolsep}{2.5pt}
% \begin{tabular}{c|ccccccc}
% % \hline
% \toprule[1.5pt]
% Method & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\ 
% % \hline
% \midrule[1pt]
% 108-dim. & 0.08x & 0.11x & 0.24x & 0.37x & 0.30x & 0.43x & \textbf{1.00x} \\ 
% 569-dim. & 0.07x & 0.05x & 0.20x & 0.26x & 0.24x & 0.38x & \textbf{1.00x} \\ 
% 1093-dim. & 0.05x & 0 & 0.14x & 0.19x & 0.19x & 0.25x & \textbf{1.00x}  \\ 
% \bottomrule[1.5pt]
% % \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

% The numerical results and detailed $P_f$ evolution are shown in  and . 
% The MC method achieves the ground truth of failure rate 2.50e-5 using 931000 simulations. 
% As shown in \Figref{case4_exp}, only after long importance sampling, are other IS-based methods able to discover the correct failure regions and their $P_f$ increases to the peak. In contrast, due to the powerful proposed pre-sampling approach, \ours discovers the correct failure regions and its $P_f$ achieves the peak right after the pre-sampling state, and it converges to the ground truth rapidly. 
% \ours achieves a fail rate of 2.49e-5 using 3400 simulations, exhibiting a relative error of 0.25\%, which outperforms others in terms of accuracy and efficiency. In comparison, MNIS, HSCS, AIS, ACS, LRTA and ASDK uses 59000, 46500, 25700, 22500, 18500 and ... simulations respectively to achieve a fail rate with the larger relative error. Compared with MNIS, \ours can achieve a up to 17.35x more accurate and 69.32x speedup. 


% \begin{figure*}
%   \centering
%   \includegraphics[width=0.75\linewidth]{exp_fig/CASE5.pdf}
%   \vspace*{-0.1in}
%   \caption{Optimal Manifold}
%   \label{SRAM_column}
%   \vspace*{-0.2in}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \vspace*{-0.1in}
%   \includegraphics[width=0.8\linewidth]{exp_fig/case5_Pfail.pdf}\\
%   \vspace{-0.1in}
%   \includegraphics[width=0.8\linewidth]{exp_fig/case5_FOM.pdf}\\
%   % \vspace{-0.1in}
%   \caption{$P_f$ and FOM on 1093-dimensional SRAM column}
%   \label{case5_exp}
%   % \vspace{-0.1in}
% \end{figure*}
\subsection{1093-Dimensional SRAM Column Circuit}

% \begin{table}
%   \vspace{-0.15in}
%   \centering
%   \caption{nOCR on 569-dimensional SRAM column}
%   \label{robustness}
%   \vspace{-0.1in}
%     \begin{adjustbox}{width=1\columnwidth,center}
%     \renewcommand\arraystretch{1.2}
%       \setlength{\tabcolsep}{2.5pt}
%       \begin{tabular}{c|cccccccc}
%         \toprule[1.5pt]
%          Method & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%         \midrule[1pt]
%          nOCR  & 74.9 & error & 202.6 & 475.4  & 528.1 & 301.8 & \bf{6855.4} \\
%         % & Mean \# of sim.      & 699000.00 & 50883.33 & 31340.00 & 15714.29 & 14071.43   & 13440.00  &  & 5300.00 \\
%          nOCR(norm) & 1.09e-2 & 0 & 2.96e-2 & 6.93e-2 & 7.70e-2 & 4.40e-2 & \bf{1} \\
%       \bottomrule[1.5pt]
%     \end{tabular}
% \end{adjustbox}
% % \vspace*{-0.1in}
% \end{table}
\cmt
{We further increase the dimensions of the problem by using a detailed BSIM5 model, learning to 1093 variation parameters.
% of the circuit our problem by adding more bit cells, leading to an even more challenging SRAM column circuit with 1093 variation parameters.
As far as we are aware, no previous published work has ever attempted to estimate the yield of such a high-dimensional problem.
% and no former researcher implements yield estimation experiment on such a high-dimensional setting. 
Similarly, the delay time of read/write is used as the output metric. }
\cmt
{We further enhance the complexity of the problem by employing an elaborate BSIM5 model, encompassing the mastery of 1093 variation parameters. To the best of our knowledge, no preceding published research has endeavored to estimate the yield of such an extensive high-dimensional quandary. Similarly, the delay time of read/write operations is utilized as the chosen output metric.}

\cmt
{We run 1,189,000 simulations using the MC method and obtain the ground-truth failure rate, 4.80e-5. The results for the competing methods are shown in \Figref{fig:1093case} and \Tabref{tab:1093}.
% The total experimental numerical results and detailed process are illustrated in \Tabref{AllCaseTable} and \Figref{case5_exp}.
The superior \ours is consistent, although this time, the improvement over the second-best method ASDK is 2.2x, not as significant as in the previous experiments. Nevertheless, the ASDK shows the largest error of 27.08\% among all methods. }
\cmt
{We conducted a total of 1,189,000 simulations utilizing MC method, leading to the derivation of the precise failure rate, which stands at 4.80e-5. The outcomes corresponding to the alternative methodologies are depicted in Figure 1 and summarized in Table 1. The supremacy of \ours remains steadfast; however, the degree of enhancement over the second-best method (ASDK) is reduced to 2.2 times, manifesting less pronounced improvement compared to our earlier experiments. It is noteworthy that ASDK exhibits the most substantial deviation, amounting to 27.08\% in terms of error, when juxtaposed against all other methods.}

\YFwrite{
We elevate the complexity of the problem by employing an intricate BSIM5 model, encompassing a mastery of 1093 variation parameters. To the best of our knowledge, no previously published research has ventured into the realm of estimating the yield for such an extensive high-dimensional challenge. In this challenging scenario, we continue to employ the delay time of read/write operations as the chosen output metric. This endeavor pushes the boundaries of yield estimation in high-dimensional contexts and underscores the need for advanced methods like \ours to tackle such complex scenarios.

We conducted a total of 1,189,000 simulations using the MC method, resulting in the precise determination of the failure rate, which stands at 4.80e-5. The results obtained using alternative methodologies are presented in Figure 1 and summarized in Table 1.
Despite the increased complexity of this high-dimensional problem, the superiority of \ours remains robust. However, the degree of improvement over the second-best method (ASDK) is somewhat reduced, with \ours showcasing a 2.2 times speedup, indicating a less pronounced enhancement compared to our earlier experiments.
It's worth noting that ASDK exhibits the most substantial deviation, with an error of 27.08\% when compared to all other methods. This underscores the robustness and consistency of \ours, even in highly complex scenarios.
}




\begin{table}[h]
\centering
\caption{Results on 1093-dimensional SRAM circuit}
\label{tab:1093}
      % \vspace*{-0.1in}
      \begin{adjustbox}{width=1\columnwidth,center}
      \renewcommand\arraystretch{1.6}
      \setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l|ccccc}
% \hline
\toprule[1.5pt]
\toprule
Method & Fail Rate & Rel. Error & \# Sim & Speedup & nACR \\ 
\midrule[1pt]
% \hline
MC & 4.80e-5 & - & 1189000 & 1x & - \\
MNIS & 4.21e-5 & 12.32\% & 81000 & 14.68x & 0.05x \\
HSCS & 1.53e-6 & N/A & 95580 & 12.44x & N/A \\
AIS & 3.79e-5 & 21.04\% & 27900 & 42.62x & 0.14x \\
ACS & 4.30e-5 & 10.42\% & 24000 & 49.54x & 0.19x \\
LRTA & 3.33e-5 & 30.63\% & 21000 & 56.61x & 0.19x \\
ASDK & 3.51e-5 & 26.87\% & 18000 & 66.05x & 0.25x \\
Proposed & \textbf{4.95e-5} & \textbf{3.13\%} & \textbf{4832} & \textbf{246.01x} & \textbf{1.00x} \\
% \hline
\bottomrule
\bottomrule[1.5pt]
\end{tabular}
\end{adjustbox}
\end{table}

\begin{figure*}
  \centering
  \begin{minipage}[t]{1\linewidth}
  \centering
  % \vspace*{-4pt}       
  \includegraphics[width=0.329\linewidth]{paper_fig/108dim.pdf}
  % \caption{108dim}
	\includegraphics[width=0.329\linewidth]{paper_fig/569dim.pdf}
 % \caption{108dim}
  \includegraphics[width=0.329\linewidth]{paper_fig/1093dim.pdf}\\
  % \vspace{-0.4in}       
  \end{minipage}
  \caption{nACR on 108, 569, 1093 dimensional SRAM Circuits}
  \label{fig:acr}
  % \vspace*{-0.2in}
\end{figure*}

% \begin{figure}[h]
% % \vspace*{-0.1in}
%   \centering
%   \includegraphics[width=0.88\linewidth]{paper_fig/1093dim.pdf}
%   % \vspace*{-0.05in}
%   \caption{nACR on 1093-dimensional SRAM circuit}
%   \label{fig:warp}
%   % \vspace*{-0.1in}
% \end{figure}

% It can be obviously concluded that \ours is still able to get the failure rate with highest accuracy and efficiency among other 6 methods, which uses merely 6400 runs of simulation and exhibits a estimated result with a 2.71\% relative error. Our method finds the correct failure region after one round of importance sampling, while other IS-based methods takes many rounds. The surrogate methods converge slower than \ours because they need a large number of training data.
% In comparison with MNIS, \ours can reach a up to 12.66x speedup and is 4.55x more accurate.

% \begin{table}
%   \centering
%       \caption{Ablation experiment of pre-sampling method}
%       \label{ablation}
%       \vspace*{-0.1in}
%       \begin{tabular}{c|c|c|c|c}
%          \midrule
%           & AIS&  AIS+  & ACS & ACS+ \\
%         \midrule
%           \# of IS & 13024 & 10854 & 12100 & 9600 \\
%           Rel. error & 7.98\% & 6.79\% & 6.59\% & 4.77\%  \\
%       \bottomrule
%     \end{tabular}
%     \vspace*{-0.15in}
%   \end{table}


\subsection{Ablation Study}
\yftodo{add serious ablation study from model 1-4 compared to normal OMSV}
% \begin{table}
%   \centering
%       \caption{Ablation experiment of pre-sampling method}
%       \label{ablation}
%       \vspace*{-0.1in}
%       \begin{tabular}{c|c|c|c|c|c|c}
%         \toprule
%            & \multicolumn{2}{|c|}{Origin method} & \multicolumn{2}{|c|}{With ours}  & \multicolumn{2}{|c}{Improvment}\\
%          \midrule
%           & Rel. error&  \# of IS  & Rel. error & \# of IS & Speedup & Acc.\\
%         \midrule
%                 AIS & 7.98\% & 13024 & 6.79\% & 10854 & & \\
%               ACS & 6.59\% & 12100 & 4.77\% & 9600 & & \\
%       \bottomrule
%     \end{tabular}
%     \vspace*{-0.15in}
%   \end{table}
% \subsection{Ablation Study}
% The onion sampling is the key contribution of this work.
\cmt{\textcolor{blue}{We validate the usefulness of the onion sampling by equipping the classic IS methods, namely, AIS and ACS ,as their pre-sampling procedure and compare with their original versions.
% their results with their original LHS sampling.
The experiments are conducted on the same 108-dimensional SRAM experiment for its fast simulation speed.
1700 samples are given for all methods as their initial sampling budget, and the results are shown in \Tabref{ablation}, which shows about 20\% improvement in accuracy speedup with our onion sampling (AIS+ and ACS+).}}
\cmt
{We substantiate the efficacy of onion sampling by integrating it into the classic IS methods, specifically AIS and ACS, in lieu of their original pre-sampling procedures. To gauge its impact, we conducted comparative experiments using the identical 108-dimensional SRAM setup, chosen for its swift simulation capabilities.

For all methods, we initiated the process with an initial sampling budget of 1700 samples. The outcomes of these experiments are detailed in \Tabref{ablation}, showcasing an approximate 20\% enhancement in accuracy speedup when leveraging our onion sampling technique (denoted as AIS+ and ACS+). This significant improvement underscores the effectiveness of our proposed approach.}

\YFwrite{
We demonstrate the effectiveness of onion sampling by incorporating it into classic IS-based methods, specifically AIS and ACS, in place of their original pre-sampling procedures. To assess its impact, we conducted comparative experiments using the same 108-dimensional SRAM setup, chosen for its rapid simulation capabilities.

For all methods, we initiate the process with an initial sampling budget of 1700 samples. The results of these experiments are detailed in Table \ref{ablation}, which shows an approximate 20\% improvement in accuracy speedup when employing our onion sampling technique (denoted as AIS+ and ACS+). This significant enhancement highlights the effectiveness of our proposed approach in enhancing the performance of traditional IS methods.
}

\begin{table}[h]
\centering
  \caption{Ablation experiment of pre-sampling method}
  \label{ablation}
  % \vspace*{-0.1in}
  \begin{adjustbox}{width=1\columnwidth,center}
    \renewcommand\arraystretch{1.5}
      \setlength{\tabcolsep}{4pt}
  \begin{tabular}{c|ccc|ccc}
    \toprule[1.3pt]
    \toprule
    & AIS & AIS+ & Impro. & ACS & ACS+ & Impro. \\
    \midrule[0.5pt]
    Rel. error & 7.98\% & 6.79\% & 1.18x & 6.59\% & 4.77\% & 1.38x  \\
    \# of IS & 13024  & 10854  & 1.20x & 12100 & 9600 & 1.26x \\
    \bottomrule
    \bottomrule[1.3pt]
  \end{tabular}
  % \vspace*{-0.2in}
  \end{adjustbox}
\end{table}


% We give both method 1000 samples to start with and let them run for 1000 iterations. \help{confirm the number of iterations}.
% 
% We can clearly see that, using hyperspherical pre-sampling AIS and ACS run 11100 and 9300 simulations to achieve the fail rate of 4.74e-5 and 5.68e-5 respectively, and that, using our proposed pre-sampling method AIS and ACS run 10030 and 8000 to achieve the fail rate of 5.31e-5 and 5.45e-5 respectively. It can be concluded that the proposed pre-sampling method does help discover promising failure regions and accelerate the speed of convergence of fail probability.
% 

% To verify the proposed pre-sampling method's contribution to the performance of \ours, we conduct the ablation experiment on the 
% ACS and AIS use the same pre-sampling algorithm, named hyperspherical pre-sampling, which draws samples on hyperspheres with increasing radius in the variation parameter space. We replace AIS and ACS's pre-sampling method with our proposed method, and implements the modified AIS and ACS on the circuit. The circuit setup is as the same as that of the Section \ref{108dim_exp}.
% To evaluate the method fairly, the modified pre-sampling procedure are fixed to run as the same number of simulation as that of the origin pre-sampling procedure.
% The real failure probability of the circuit is set as 5.01e-5. 



\subsection{{Robustness Study}}
\cmt{\textcolor{blue}{To further assess the robustness of our method, we conduct a robustness study on the 108-dimensional SRAM circuit by running experiments 10 times with random initializations. The final estimations with relative errors larger than 50\% are marked fail. The statistical results for successful runs are shown in \Tabref{tab:robust}. As we expect, the surrogate methods, LRTA and ASDK, suffer from great instability with more than 5 times fail, whereas the IS methods are more stable. In contrast, \ours shows the best performance for all metrics.}}

\YFwrite{
For a comprehensive evaluation of the robustness of our methodology, we undertake an in-depth robustness study on the three dimensional SRAM circuits. This entails running experiments a total of 10 times, each with distinct random initializations. In our analysis, estimations that exhibit relative errors surpassing 50\% are deemed failures, and these are duly marked as such. The statistical outcomes for the successful runs are delineated in \Tabref{tab:robust}.

In the 108-dimensional SRAM circuit experiment, as anticipated, the surrogate techniques, namely, LRTA and ASDK, exhibit pronounced instability, resulting in failure rates exceeding 5 times. In stark contrast, the IS methods demonstrate a higher degree of stability. Notably, \ours emerges as the superior performer across all metrics, showcasing its resilience and effectiveness even under such rigorous testing conditions.

In the 569-dimensional SRAM circuit experiment

In the 1093-dimensional SRAM circuit experiment
}


\begin{table*}[ht]
\centering
\caption{Robustness Test results on three SRAM column circuits}
      \label{tab:robust}
      % \vspace*{-0.1in}
      \begin{adjustbox}{width=2\columnwidth,center}
      \renewcommand\arraystretch{1.6}
      \setlength{\tabcolsep}{5.5pt}
\begin{tabular}{l|ccc|ccc|ccc}
% \hline
\toprule[1.5pt]
\toprule
 & \multicolumn{3}{c|}{108-dimensional Case} & \multicolumn{3}{c|}{569-dimensional Case} & \multicolumn{3}{c}{1093-dimensional Case} \\ 
 % \hline
 \midrule
Method & Rel. Error & Speedup & \# Fail & Rel. Error & Speedup & \# Fail & Rel. Error & Speedup & \# Fail \\ 
% \hline
\midrule[1pt]
MNIS & 12.57\% & 34.84x & 2/10 & 20.40\% & 23.12x & 4/10 & 36.67\% & 21.32x & 4/10 \\
HSCS & 35.28\% & 20.72x & 6/10 & 45.78\% & 12.93x & 8/10 & N/A & N/A & 10/10 \\
AIS & 23.73\% & 41.35x & 2/10 & 10.14\% & 36.94x & 4/10 & 26.62\% & 42.91x & 5/10 \\
ACS & 10.96\% & 54.45x & 2/10 & 16.45\% & 44.38x & 5/10 & 12.50\% & 50.76x & 5/10 \\
LRTA & 22.95\% & 55.92x & 2/10 & 20.40\% & 52.15x & 5/10 & 21.50\% & 45.15x & 6/10 \\
ASDK & 15.31\% & 79.35x & 5/10 & 17.85\% & 87.21x & 5/10 & 30.18\% & 84.98x & 7/10 \\
Proposed & \textbf{1.91\%} & \textbf{131.89x} & \textbf{1/10} & \textbf{1.91\%} & \textbf{131.89x} & \textbf{2/10} & \textbf{1.91\%} & \textbf{131.89x} & \textbf{3/10} \\ 
% \hline
\bottomrule
\bottomrule[1.5pt]
\end{tabular}
\end{adjustbox}
\end{table*}


% \help{what is the final estimation?}
% \vspace{-0.2in}
% \begin{table}
%   \vspace{-0.15in}
%   \centering
%   \caption{Robustness test on 108-dimensional SRAM column}
%   \label{robustness}
%   \vspace{-0.1in}
%     \begin{adjustbox}{width=1\columnwidth,center}
%       \begin{tabular}{c|cccccccc}
%         \toprule
%          Method & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%         \midrule
%          Avg. RE  & 16.00\% & 8.90\% & 6.64\% & 6.45\%  & 12.85\% & 10.18\% & \bf{1.91\%} \\
%         % & Mean \# of sim.      & 699000.00 & 50883.33 & 31340.00 & 15714.29 & 14071.43   & 13440.00  &  & 5300.00 \\
%          Avg. speedup & 13.73x & 22.30x & 44.48x & 49.68x & 52.01x & 75.98x & \bf{131.89x} \\
%        \midrule
%         \# Fail & 4/10 & 4/10 & 3/10 & 3/10 & 5/10 & 9/10 & \bf{1/10} \\
%       \bottomrule
%     \end{tabular}
% \end{adjustbox}
% \vspace*{-0.2in}
% \end{table}
  

% \begin{table*}
%   \centering
%       \caption{Numerical results on 108-dimensional SRAM column}
%       \begin{tabular}{c|c|cccccccc}
%         \toprule
%          & Results & MC & MNIS & HSCS & AIS & ACS & LRTA & ASDK & Proposed \\
%         \midrule
        
%         \multirow{2}{*}{Successful runs} 
%         % & Mean failure prob.   & 5.01e-5 & 4.21e-5 & 4.56e-05 & 4.67e-5 & 5.33e-5  & 4.37e-05 &  & 5.10e-5 \\
%         & Mean relative error  & - & 16.00\% & 8.90\% & 6.64\% & 6.45\%  & 12.85\% & 10.18\% & 1.91\% \\
%         % & Mean \# of sim.      & 699000.00 & 50883.33 & 31340.00 & 15714.29 & 14071.43   & 13440.00  &  & 5300.00 \\
%         & Mean speedup & 1x & 13.73x & 22.30x & 44.48x & 49.68x & 52.01x & 75.98x & 131.89x \\
%        \midrule
      
%        \multirow{1}{*}{Failed runs} 
%         & Failed times & N/A & 4/10 & 4/10 & 3/10 & 3/10 & 5/10 & 9/10 & 1/10 \\
%       \bottomrule
%     \end{tabular}
%   \end{table*}
  
